FastSTMF: Efficient tropical matrix factorization algorithm for sparse data

Matrix factorization, one of the most popular methods in machine learning, has recently benefited from introducing non-linearity in prediction tasks using tropical semiring. The non-linearity enables a better fit to extreme values and distributions, thus discovering high-variance patterns that differ from those found by standard linear algebra. However, the optimization process of various tropical matrix factorization methods is slow. In our work, we propose a new method FastSTMF based on Sparse Tropical Matrix Factorization (STMF), which introduces a novel strategy for updating factor matrices that results in efficient computational performance. We evaluated the efficiency of FastSTMF on synthetic and real gene expression data from the TCGA database, and the results show that FastSTMF outperforms STMF in both accuracy and running time. Compared to NMF, we show that FastSTMF performs better on some datasets and is not prone to overfitting as NMF. This work sets the basis for developing other matrix factorization techniques based on many other semirings using a new proposed optimization process.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> main_backmatter.tex <==
\textbf{Amra Omanović} received a master's degree from the Faculty of Computer and Information Science, University of Ljubljana, in 2018. She is a junior researcher at the Faculty of Computer and Information Science, University of Ljubljana. Her research is focused on the application of linear algebra over semirings in data embedding and fusion methods.

\textbf{Polona Oblak} received the doctoral degree from the Faculty of Mathematics and Physics, University of Ljubljana, in 2008. She is an associate professor at the Faculty of Computer and Information Science, University of Ljubljana. Her research interests include inverse eigenvalue problems for graphs, linear algebra over semirings and combinatorial matrix theory.

\textbf{Tomaž Curk} received a doctoral degree from the Faculty of Computer and Information Science, University of Ljubljana, in 2007. He is an associate professor and serves as a vice-dean for research at the Faculty of Computer and Information Science, University of Ljubljana. His research is focused on the application of machine learning and data integration methods in bioinformatics.
